An identity involving $h$-polynomials of poset associahedra and type B Narayana polynomials

For any finite connected poset $P$, Galashin introduced a simple convex $(|P|-2)$-dimensional polytope $\mathscr{A}(P)$ called the poset associahedron. Let $P$ be a poset with a proper autonomous subposet $S$ that is a chain of size $n$. For $1\leq i \leq n$, let $P_i$ be the poset obtained from $P$ by replacing $S$ by an antichain of size $i$. We show that the $h$-polynomial of $\mathscr{A}(P)$ can be written in terms of the $h$-polynomials of $\mathscr{A}(P_i)$ and type B Narayana polynomials. We then use the identity to deduce several identities involving Narayana polynomials, Eulerian polynomials, and stack-sorting preimages.

==> tikz.tex <==
% \newcommand{\convexpath}[2]{
%   [   
%   create hullcoords/.code={
%     \global\edef\namelist{#1}
%     \foreach [count=\counter] \nodename in \namelist {
%       \global\edef\numberofnodes{\counter}
%       \coordinate (hullcoord\counter) at (\nodename);
%     }
%     \coordinate (hullcoord0) at (hullcoord\numberofnodes);
%     \pgfmathtruncatemacro\lastnumber{\numberofnodes+1}
%     \coordinate (hullcoord\lastnumber) at (hullcoord1);
%   },
%   create hullcoords
%   ]
%   ($(hullcoord1)!#2!-90:(hullcoord0)$)
%   \foreach [
%   evaluate=\currentnode as \previousnode using \currentnode-1,
%   evaluate=\currentnode as \nextnode using \currentnode+1
%   ] \currentnode in {1,...,\numberofnodes} {
%     let \p1 = ($(hullcoord\currentnode) - (hullcoord\previousnode)$),
%     \n1 = {atan2(\y1,\x1) + 90},
%     \p2 = ($(hullcoord\nextnode) - (hullcoord\currentnode)$),
%     \n2 = {atan2(\y2,\x2) + 90},
%     \n{delta} = {Mod(\n2-\n1,360) - 360}
%     in 
%     {arc [start angle=\n1, delta angle=\n{delta}, radius=#2]}
%     -- ($(hullcoord\nextnode)!#2!-90:(hullcoord\currentnode)$) 
%   }
% }



%%%% -------------------------------------------- %%%%%

% tubingEx

% \node (v1) [fill = white,circle,scale=1,anchor=center] at (0,0) {1};
% \node (v2) [fill = white,circle,scale=1,anchor=center] at (-1,1) {2};
% \node (v3) [fill = white,circle,scale=1,anchor=center] at (0,1) {3};
% \node (v4) [fill = white,circle,scale=1,anchor=center] at (1,1) {4};
% \node (v5) [fill = white,circle,scale=1,anchor=center] at (0,2) {5};

% \draw[black] (v1) -- (v2);
% \draw[black] (v1) -- (v3);
% \draw[black] (v1) -- (v4);
% \draw[black] (v5) -- (v2);
% \draw[black] (v5) -- (v3);
% \draw[black] (v5) -- (v4);

% \draw[red] \convexpath{v1,v2,v3}{0.25cm};
% \draw[red] \convexpath{v4,v5}{0.25cm};


% \node (t1) [fill = white,circle,scale=1,anchor=center] at (4,0) {1};
% \node (t2) [fill = white,circle,scale=1,anchor=center] at (2.5,2) {2};
% \node (t3) [fill = white,circle,scale=1,anchor=center] at (3.5,2) {3};
% \node (t4) [fill = white,circle,scale=1,anchor=center] at (4.5,2) {4};
% \node (t5) [fill = white,circle,scale=1,anchor=center] at (5.5,2) {5};

% \draw[black] (t1) -- (t2);
% \draw[black] (t1) -- (t3);
% \draw[black] (t1) -- (t4);
% \draw[black] (t1) -- (t5);

% \draw[red] \convexpath{t4,t1,t3}{0.25cm};
% \draw[red] \convexpath{t5,t1,t3}{0.45cm};


% \node (s1) [fill = white,circle,scale=1,anchor=center] at (7.5,0) {1};
% \node (s2) [fill = white,circle,scale=1,anchor=center] at (7.5,2) {2};
% \node (s3) [fill = white,circle,scale=1,anchor=center] at (9.5,0) {3};
% \node (s4) [fill = white,circle,scale=1,anchor=center] at (9.5,2) {4};
% \node (s5) [fill = white,circle,scale=1,anchor=center] at (11.5,0) {5};
% \node (s6) [fill = white,circle,scale=1,anchor=center] at (11.5,2) {6};

% \draw[black] (s1) -- (s2);
% \draw[black] (s3) -- (s2);
% \draw[black] (s3) -- (s4);
% \draw[black] (s5) -- (s4);
% \draw[black] (s5) -- (s6);
% \draw[black] (s1) -- (s6);

% \draw[red] \convexpath{s4,s3,s2}{0.25cm};
% \draw[red] \convexpath{s5,s6}{0.25cm};
% \draw[red] \convexpath{s6,s5,s3,s2}{0.45cm};





%%%% -------------------------------------------- %%%%%

% tubingNonEx


% \node (v1) [fill = white,circle,scale=1,anchor=center] at (0,0) {1};
% \node (v2) [fill = white,circle,scale=1,anchor=center] at (-1,1) {2};
% \node (v3) [fill = white,circle,scale=1,anchor=center] at (0,1) {3};
% \node (v4) [fill = white,circle,scale=1,anchor=center] at (1,1) {4};
% \node (v5) [fill = white,circle,scale=1,anchor=center] at (0,2) {5};

% \draw[black] (v1) -- (v2);
% \draw[black] (v1) -- (v3);
% \draw[black] (v1) -- (v4);
% \draw[black] (v5) -- (v2);
% \draw[black] (v5) -- (v3);
% \draw[black] (v5) -- (v4);

% \draw[red] \convexpath{v1,v2,v3}{0.25cm};
% \draw[red] \convexpath{v3,v5}{0.25cm};


% \node (t1) [fill = white,circle,scale=1,anchor=center] at (4,0) {1};
% \node (t2) [fill = white,circle,scale=1,anchor=center] at (2.5,2) {2};
% \node (t3) [fill = white,circle,scale=1,anchor=center] at (3.5,2) {3};
% \node (t4) [fill = white,circle,scale=1,anchor=center] at (4.5,2) {4};
% \node (t5) [fill = white,circle,scale=1,anchor=center] at (5.5,2) {5};

% \draw[black] (t1) -- (t2);
% \draw[black] (t1) -- (t3);
% \draw[black] (t1) -- (t4);
% \draw[black] (t1) -- (t5);

% \draw[red] \convexpath{t4,t1,t3}{0.25cm};
% \draw[red] \convexpath{t5,t1}{0.25cm};


% \node (s1) [fill = white,circle,scale=1,anchor=center] at (7.5,0) {1};
% \node (s2) [fill = white,circle,scale=1,anchor=center] at (7.5,2) {2};
% \node (s3) [fill = white,circle,scale=1,anchor=center] at (9.5,0) {3};
% \node (s4) [fill = white,circle,scale=1,anchor=center] at (9.5,2) {4};
% \node (s5) [fill = white,circle,scale=1,anchor=center] at (11.5,0) {5};
% \node (s6) [fill = white,circle,scale=1,anchor=center] at (11.5,2) {6};

% \draw[black] (s1) -- (s2);
% \draw[black] (s3) -- (s2);
% \draw[black] (s3) -- (s4);
% \draw[black] (s5) -- (s4);
% \draw[black] (s5) -- (s6);
% \draw[black] (s1) -- (s6);

% \draw[red] \convexpath{s1,s2}{0.25cm};
% \draw[red] \convexpath{s3,s4}{0.25cm};
% \draw[red] \convexpath{s5,s6}{0.25cm};








%%%% -------------------------------------------- %%%%%

% posetExPerm


% \definecolor{lightblue}{rgb}{0.8, 1.0, 1.0}
% \definecolor{lightyellow}{rgb}{1.0, 1.0, 0.8}

% \coordinate (a) at (0,0);
% \coordinate (b) at (8,0);
% \coordinate (c) at (12,{4*sqrt(3)});
% \coordinate (d) at (8,{8*sqrt(3)});
% \coordinate (e) at (0,{8*sqrt(3)});
% \coordinate (f) at (-4,{4*sqrt(3)});
% \draw[black, line width = 2mm, fill = lightblue] (a) -- (b) -- (c) -- (d) -- (e) -- (f) -- cycle;



% \coordinate (s0) at (0,-1);
% \coordinate (s1) at (-2,1);
% \coordinate (s2) at (0,1);
% \coordinate (s3) at (2,1);

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s0) -- (s2);
% \draw[black] (s0) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s1}{0.3cm};
% \draw[red,rounded corners = 4mm] (0,-1.6) -- (2.6,1) -- (2,1.6) -- (0,-0.4) -- (-2,1.6) -- (-2.6,1) -- cycle;




% \coordinate (s0) at (8,-1);
% \coordinate (s1) at (6,1);
% \coordinate (s2) at (8,1);
% \coordinate (s3) at (10,1);

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s0) -- (s2);
% \draw[black] (s0) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s3}{0.3cm};
% \draw[red,rounded corners = 4mm] (8,-1.6) -- (10.6,1) -- (10,1.6) -- (8,-0.4) -- (6,1.6) -- (5.4,1) -- cycle;




% \coordinate (s0) at (12,{4*sqrt(3)-1});
% \coordinate (s1) at (10,{4*sqrt(3)+1});
% \coordinate (s2) at (12,{4*sqrt(3)+1});
% \coordinate (s3) at (14,{4*sqrt(3)+1});

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s0) -- (s2);
% \draw[black] (s0) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s3}{0.3cm};
% \draw[red] \convexpath{s2,s3,s0}{0.4cm};




% \coordinate (s0) at (8,{8*sqrt(3)-1});
% \coordinate (s1) at (6,{8*sqrt(3)+1});
% \coordinate (s2) at (8,{8*sqrt(3)+1});
% \coordinate (s3) at (10,{8*sqrt(3)+1});

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s0) -- (s2);
% \draw[black] (s0) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s2}{0.3cm};
% \draw[red] \convexpath{s2,s3,s0}{0.4cm};




% \coordinate (s0) at (0,{8*sqrt(3)-1});
% \coordinate (s1) at (-2,{8*sqrt(3)+1});
% \coordinate (s2) at (0,{8*sqrt(3)+1});
% \coordinate (s3) at (2,{8*sqrt(3)+1});

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s0) -- (s2);
% \draw[black] (s0) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s2}{0.3cm};
% \draw[red] \convexpath{s1,s2,s0}{0.4cm};




% \coordinate (s0) at (-4,{4*sqrt(3)-1});
% \coordinate (s1) at (-6,{4*sqrt(3)+1});
% \coordinate (s2) at (-4,{4*sqrt(3)+1});
% \coordinate (s3) at (-2,{4*sqrt(3)+1});

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s0) -- (s2);
% \draw[black] (s0) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s1}{0.3cm};
% \draw[red] \convexpath{s1,s2,s0}{0.4cm};







%%%% -------------------------------------------- %%%%%

% posetExAss



% \definecolor{lightblue}{rgb}{0.8, 1.0, 1.0}
% \definecolor{lightyellow}{rgb}{1.0, 1.0, 0.8}

% \coordinate (a) at (0,0);
% \coordinate (b) at (8,0);
% \coordinate (c) at ({8+8*cos(72)},{8*sin(72)});
% \coordinate (d) at (4,{4*tan(72)});
% \coordinate (e) at ({-8*cos(72)},{8*sin(72)});
% \draw[black, line width = 2mm, fill = lightblue] (a) -- (b) -- (c) -- (d) -- (e) -- cycle;



% \coordinate (s0) at (0,-3);
% \coordinate (s1) at (0,-1);
% \coordinate (s2) at (0,1);
% \coordinate (s3) at (0,3);

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s1}{0.3cm};
% \draw[red] \convexpath{s2,s3}{0.3cm};




% \coordinate (s0) at (8,-3);
% \coordinate (s1) at (8,-1);
% \coordinate (s2) at (8,1);
% \coordinate (s3) at (8,3);

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s1,s3}{0.4cm};
% \draw[red] \convexpath{s2,s3}{0.3cm};




% \coordinate (s0) at ({8+8*cos(72)},{8*sin(72)-3});
% \coordinate (s1) at ({8+8*cos(72)},{8*sin(72)-1});
% \coordinate (s2) at ({8+8*cos(72)},{8*sin(72)+1});
% \coordinate (s3) at ({8+8*cos(72)},{8*sin(72)+3});

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s1,s3}{0.4cm};
% \draw[red] \convexpath{s1,s2}{0.3cm};




% \coordinate (s0) at (4,{4*tan(72)-3});
% \coordinate (s1) at (4,{4*tan(72)-1});
% \coordinate (s2) at (4,{4*tan(72)+1});
% \coordinate (s3) at (4,{4*tan(72)+3});

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s2}{0.4cm};
% \draw[red] \convexpath{s1,s2}{0.3cm};




% \coordinate (s0) at ({-8*cos(72)},{8*sin(72)-3});
% \coordinate (s1) at ({-8*cos(72)},{8*sin(72)-1});
% \coordinate (s2) at ({-8*cos(72)},{8*sin(72)+1});
% \coordinate (s3) at ({-8*cos(72)},{8*sin(72)+3});

% \draw[lightyellow, fill = lightyellow] \convexpath{s0,s1,s3}{0.5cm};

% \draw[black] (s0) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s0) {0};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s0,s2}{0.4cm};
% \draw[red] \convexpath{s0,s1}{0.3cm};












%%%% -------------------------------------------- %%%%%

% graphExPerm



% \definecolor{lightblue}{rgb}{0.8, 1.0, 1.0}
% \definecolor{lightyellow}{rgb}{1.0, 1.0, 0.8}

% \coordinate (a) at (0,0);
% \coordinate (b) at (8,0);
% \coordinate (c) at (12,{4*sqrt(3)});
% \coordinate (d) at (8,{8*sqrt(3)});
% \coordinate (e) at (0,{8*sqrt(3)});
% \coordinate (f) at (-4,{4*sqrt(3)});
% \draw[black, line width = 2mm, fill = lightblue] (a) -- (b) -- (c) -- (d) -- (e) -- (f) -- cycle;



% \coordinate (s1) at ({-sqrt(3)*3/4},-0.75);
% \coordinate (s2) at ({sqrt(3)*3/4},-0.75);
% \coordinate (s3) at (0,1.5);

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3,s2}{0.5cm};

% \draw[black] (s3) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s1,s3}{0.4cm};
% \draw (s1) [red] circle (0.3cm) [fill=none];
    



% \coordinate (s1) at ({8-sqrt(3)*3/4},-0.75);
% \coordinate (s2) at ({8+sqrt(3)*3/4},-0.75);
% \coordinate (s3) at (8,1.5);

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3,s2}{0.5cm};

% \draw[black] (s3) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s1,s3}{0.4cm};
% \draw (s3) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at ({12-sqrt(3)*3/4},{4*sqrt(3)-0.75});
% \coordinate (s2) at ({12+sqrt(3)*3/4},{4*sqrt(3)-0.75});
% \coordinate (s3) at (12,{4*sqrt(3)+1.5});

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3,s2}{0.5cm};

% \draw[black] (s3) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s2,s3}{0.4cm};
% \draw (s3) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at ({8-sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s2) at ({8+sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s3) at (8,{8*sqrt(3)+1.5});

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3,s2}{0.5cm};

% \draw[black] (s3) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s2,s3}{0.4cm};
% \draw (s2) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at ({0-sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s2) at ({0+sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s3) at (0,{8*sqrt(3)+1.5});

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3,s2}{0.5cm};

% \draw[black] (s3) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s2,s1}{0.4cm};
% \draw (s2) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at ({-4-sqrt(3)*3/4},{4*sqrt(3)-0.75});
% \coordinate (s2) at ({-4+sqrt(3)*3/4},{4*sqrt(3)-0.75});
% \coordinate (s3) at (-4,{4*sqrt(3)+1.5});

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3,s2}{0.5cm};

% \draw[black] (s3) -- (s1);
% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s2,s1}{0.4cm};
% \draw (s1) [red] circle (0.3cm) [fill=none];












%%%% -------------------------------------------- %%%%%

% graphExAss




% \definecolor{lightblue}{rgb}{0.8, 1.0, 1.0}
% \definecolor{lightyellow}{rgb}{1.0, 1.0, 0.8}

% \coordinate (a) at (0,0);
% \coordinate (b) at (8,0);
% \coordinate (c) at ({8+8*cos(72)},{8*sin(72)});
% \coordinate (d) at (4,{4*tan(72)});
% \coordinate (e) at ({-8*cos(72)},{8*sin(72)});
% \draw[black, line width = 2mm, fill = lightblue] (a) -- (b) -- (c) -- (d) -- (e) -- cycle;



% \coordinate (s1) at (0,-2);
% \coordinate (s2) at (0,0);
% \coordinate (s3) at (0,2);

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3}{0.5cm};

% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw (s1) [red] circle (0.3cm) [fill=none];
% \draw (s3) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at (8,-2);
% \coordinate (s2) at (8,0);
% \coordinate (s3) at (8,2);

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3}{0.5cm};

% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s2,s3}{0.4cm};
% \draw (s3) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at ({8+8*cos(72)},{8*sin(72)-2});
% \coordinate (s2) at ({8+8*cos(72)},{8*sin(72)});
% \coordinate (s3) at ({8+8*cos(72)},{8*sin(72)+2});

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3}{0.5cm};

% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s2,s3}{0.4cm};
% \draw (s2) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at (4,{4*tan(72)-2});
% \coordinate (s2) at (4,{4*tan(72)});
% \coordinate (s3) at (4,{4*tan(72)+2});

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3}{0.5cm};

% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s1,s2}{0.4cm};
% \draw (s2) [red] circle (0.3cm) [fill=none];




% \coordinate (s1) at ({-8*cos(72)},{8*sin(72)-2});
% \coordinate (s2) at ({-8*cos(72)},{8*sin(72)});
% \coordinate (s3) at ({-8*cos(72)},{8*sin(72)+2});

% \draw[lightyellow, fill = lightyellow] \convexpath{s1,s3}{0.5cm};

% \draw[black] (s1) -- (s2);
% \draw[black] (s2) -- (s3);

% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s1) {1};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s2) {2};
% \node [fill = lightyellow, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[red] \convexpath{s1,s2}{0.4cm};
% \draw (s1) [red] circle (0.3cm) [fill=none];











%%%% -------------------------------------------- %%%%%

% graphTubingEx




% \node (v1) [fill = white,circle,scale=1,anchor=center] at (0,0) {1};
% \node (v2) [fill = white,circle,scale=1,anchor=center] at (-1,1) {2};
% \node (v3) [fill = white,circle,scale=1,anchor=center] at (1,1) {3};
% \node (v4) [fill = white,circle,scale=1,anchor=center] at (0,2) {4};

% \draw[black] (v1) -- (v2);
% \draw[black] (v2) -- (v4);
% \draw[black] (v3) -- (v4);
% \draw[black] (v4) -- (v1);
% \draw[black] (v1) -- (v3);

% \draw[red] \convexpath{v1,v2,v3}{0.35cm};
% \draw (v2) [red] circle (0.25cm) [fill=none];
% \draw (v3) [red] circle (0.25cm) [fill=none];


% \node (t1) [fill = white,circle,scale=1,anchor=center] at (2.5,1) {1};
% \node (t2) [fill = white,circle,scale=1,anchor=center] at (3.5,1) {2};
% \node (t3) [fill = white,circle,scale=1,anchor=center] at (4.5,1) {3};
% \node (t4) [fill = white,circle,scale=1,anchor=center] at (5.5,1) {4};

% \draw[black] (t1) -- (t2);
% \draw[black] (t2) -- (t3);
% \draw[black] (t4) -- (t3);

% \draw[red] \convexpath{t1,t3}{0.35cm};
% \draw[red] \convexpath{t2,t3}{0.25cm};


% \node (s1) [fill = white,circle,scale=1,anchor=center] at (7,0) {1};
% \node (s2) [fill = white,circle,scale=1,anchor=center] at (7,2) {2};
% \node (s3) [fill = white,circle,scale=1,anchor=center] at (9,2) {3};
% \node (s4) [fill = white,circle,scale=1,anchor=center] at (9,0) {4};

% \draw[black] (s1) -- (s2);
% \draw[black] (s3) -- (s2);
% \draw[black] (s3) -- (s4);
% \draw[black] (s1) -- (s4);

% \draw (s1) [red] circle (0.25cm) [fill=none];
% \draw (s3) [red] circle (0.25cm) [fill=none];










%%%% -------------------------------------------- %%%%%

% graphTubingNonEx


% \node (v1) [fill = white,circle,scale=1,anchor=center] at (0,0) {1};
% \node (v2) [fill = white,circle,scale=1,anchor=center] at (-1,1) {2};
% \node (v3) [fill = white,circle,scale=1,anchor=center] at (1,1) {3};
% \node (v4) [fill = white,circle,scale=1,anchor=center] at (0,2) {4};

% \draw[black] (v1) -- (v2);
% \draw[black] (v2) -- (v4);
% \draw[black] (v3) -- (v4);
% \draw[black] (v4) -- (v1);
% \draw[black] (v1) -- (v3);

% \draw (v1) [red] circle (0.25cm) [fill=none];
% \draw (v4) [red] circle (0.25cm) [fill=none];


% \node (t1) [fill = white,circle,scale=1,anchor=center] at (2.5,1) {1};
% \node (t2) [fill = white,circle,scale=1,anchor=center] at (3.5,1) {2};
% \node (t3) [fill = white,circle,scale=1,anchor=center] at (4.5,1) {3};
% \node (t4) [fill = white,circle,scale=1,anchor=center] at (5.5,1) {4};

% \draw[black] (t1) -- (t2);
% \draw[black] (t2) -- (t3);
% \draw[black] (t4) -- (t3);

% \draw[red] \convexpath{t1,t3}{0.35cm};
% \draw[red] \convexpath{t4,t3}{0.25cm};


% \node (s1) [fill = white,circle,scale=1,anchor=center] at (7,0) {1};
% \node (s2) [fill = white,circle,scale=1,anchor=center] at (7,2) {2};
% \node (s3) [fill = white,circle,scale=1,anchor=center] at (9,2) {3};
% \node (s4) [fill = white,circle,scale=1,anchor=center] at (9,0) {4};

% \draw[black] (s1) -- (s2);
% \draw[black] (s3) -- (s2);
% \draw[black] (s3) -- (s4);
% \draw[black] (s1) -- (s4);

% \draw (s1) [red] circle (0.25cm) [fill=none];
% \draw[red] \convexpath{s4,s3}{0.25cm};









%%%% -------------------------------------------- %%%%%

% ss-ex



% \draw[black] (0,5) -- (0,2);
% \draw[black] (1,2) -- (0,2);
% \draw[black] (1,5) -- (1,2);


% \draw (0.5,1.5) node[anchor=center, scale = 1.5] {stack};
% \draw (1.2,5.5) node[anchor=west, scale = 1.5] {$3~~1~~4~~2$};



% \draw[black] (6,5) -- (6,2);
% \draw[black] (7,2) -- (6,2);
% \draw[black] (7,5) -- (7,2);

% \draw (6.5,2.5) node[anchor=center, scale = 1.5] {$3$};
% \draw (6.5,1.5) node[anchor=center, scale = 1.5] {stack};
% \draw (7.2,5.5) node[anchor=west, scale = 1.5] {$1~~4~~2$};



% \draw[black] (12,5) -- (12,2);
% \draw[black] (13,2) -- (12,2);
% \draw[black] (13,5) -- (13,2);

% \draw (12.5,2.5) node[anchor=center, scale = 1.5] {$3$};
% \draw (12.5,3.5) node[anchor=center, scale = 1.5] {$1$};
% \draw (12.5,1.5) node[anchor=center, scale = 1.5] {stack};
% \draw (13.2,5.5) node[anchor=west, scale = 1.5] {$4~~2$};



% \draw[black] (18,5) -- (18,2);
% \draw[black] (19,2) -- (18,2);
% \draw[black] (19,5) -- (19,2);

% \draw (18.5,2.5) node[anchor=center, scale = 1.5] {$3$};
% \draw (18.5,1.5) node[anchor=center, scale = 1.5] {stack};
% \draw (19.2,5.5) node[anchor=west, scale = 1.5] {$4~~2$};
% \draw (17.8,5.5) node[anchor=east, scale = 1.5] {$1$};



% \draw[black] (24,5) -- (24,2);
% \draw[black] (25,2) -- (24,2);
% \draw[black] (25,5) -- (25,2);

% \draw (24.5,1.5) node[anchor=center, scale = 1.5] {stack};
% \draw (25.2,5.5) node[anchor=west, scale = 1.5] {$4~~2$};
% \draw (23.8,5.5) node[anchor=east, scale = 1.5] {$1~~3$};



% \draw[black] (3,0) -- (3,-3);
% \draw[black] (4,-3) -- (3,-3);
% \draw[black] (4,0) -- (4,-3);

% \draw (3.5,-2.5) node[anchor=center, scale = 1.5] {$4$};
% \draw (3.5,-3.5) node[anchor=center, scale = 1.5] {stack};
% \draw (4.2,0.5) node[anchor=west, scale = 1.5] {$2$};
% \draw (2.8,0.5) node[anchor=east, scale = 1.5] {$1~~3$};



% \draw[black] (9,0) -- (9,-3);
% \draw[black] (10,-3) -- (9,-3);
% \draw[black] (10,0) -- (10,-3);

% \draw (9.5,-2.5) node[anchor=center, scale = 1.5] {$4$};
% \draw (9.5,-1.5) node[anchor=center, scale = 1.5] {$2$};
% \draw (9.5,-3.5) node[anchor=center, scale = 1.5] {stack};
% \draw (8.8,0.5) node[anchor=east, scale = 1.5] {$1~~3$};



% \draw[black] (15,0) -- (15,-3);
% \draw[black] (16,-3) -- (15,-3);
% \draw[black] (16,0) -- (16,-3);

% \draw (15.5,-2.5) node[anchor=center, scale = 1.5] {$4$};
% \draw (15.5,-3.5) node[anchor=center, scale = 1.5] {stack};
% \draw (14.8,0.5) node[anchor=east, scale = 1.5] {$1~~3~~2$};



% \draw[black] (21,0) -- (21,-3);
% \draw[black] (22,-3) -- (21,-3);
% \draw[black] (22,0) -- (22,-3);

% \draw (22.5,-3.5) node[anchor=center, scale = 1.5] {stack};
% \draw (21.8,0.5) node[anchor=east, scale = 1.5] {$1~~3~~2~~4$};







%%%% -------------------------------------------- %%%%%

% reading-order-ex


% \node (v1) [fill = white,circle,scale=1,anchor=center] at (9,5) {1};
% \node (v2) [fill = white,circle,scale=1,anchor=center] at (10,6) {2};
% \node (v3) [fill = white,circle,scale=1,anchor=center] at (6,6) {3};
% \node (v4) [fill = white,circle,scale=1,anchor=center] at (7,7) {4};
% \node (v5) [fill = white,circle,scale=1,anchor=center] at (8,6) {5};
% \node (v6) [fill = white,circle,scale=1,anchor=center] at (9,7) {6};
% \node (v7) [fill = white,circle,scale=1,anchor=center] at (8,8) {7};


% \draw[black] (v7) -- (v6);
% \draw[black] (v7) -- (v4);
% \draw[black] (v5) -- (v6);
% \draw[black] (v2) -- (v6);
% \draw[black] (v1) -- (v2);
% \draw[black] (v4) -- (v3);



% \node (w1) [fill = white,circle,scale=1,anchor=center] at (3,6.5) {3475612};

% \node (w2) [fill = white,circle,scale=1,anchor=center] at (13,6.5) {3451267};

% \draw[-Stealth, black] (5.5,6.5) -- (w1);

% \draw[-Stealth, black] (10.5,6.5) -- (w2);


% \node (w1) [circle,scale=1,anchor=center] at (4.5,6.75) {$\mathcal{I}$};

% \node (w2) [circle,scale=1,anchor=center] at (11.5,6.75) {$\mathcal{P}$};









%%%% -------------------------------------------- %%%%%

% bt-dyck-bij


% \node (v1) [fill = black, circle, scale=0.5, anchor=center] at (2,9) {};
% \node (v2) [fill = black, circle, scale=0.5, anchor=center] at (1,8) {};
% \node (v3) [fill = black, circle, scale=0.5, anchor=center] at (3,8) {};
% \node (v4) [fill = black, circle, scale=0.5, anchor=center] at (1.5,7) {};

% \draw[black] (v1) -- (v2);
% \draw[black] (v1) -- (v3);
% \draw[black] (v4) -- (v2);


% \draw[-Stealth, black] (4,7.5) -- (5.5,7.5);


% \node (v1) [fill = black, circle, scale=0.5, anchor=center] at (8,9) {};
% \node (v2) [fill = black, circle, scale=0.5, anchor=center] at (7,8) {};
% \node (v3) [fill = black, circle, scale=0.5, anchor=center] at (9,8) {};
% \node (v4) [fill = black, circle, scale=0.5, anchor=center] at (7.5,7) {};
% \node (v5) [fill = red, circle, scale=0.5, anchor=center] at (6.5,7) {};
% \node (v6) [fill = red, circle, scale=0.5, anchor=center] at (7,6) {};
% \node (v7) [fill = red, circle, scale=0.5, anchor=center] at (8,6) {};
% \node (v8) [fill = red, circle, scale=0.5, anchor=center] at (8.5,7) {};
% \node (v9) [fill = red, circle, scale=0.5, anchor=center] at (9.5,7) {};

% \draw[black] (v1) -- (v2);
% \draw[black] (v1) -- (v3);
% \draw[black] (v4) -- (v2);
% \draw[black] (v2) -- (v5);
% \draw[black] (v4) -- (v6);
% \draw[black] (v4) -- (v7);
% \draw[black] (v3) -- (v8);
% \draw[black] (v3) -- (v9);


% \draw[-Stealth, black] (10.5,7.5) -- (12,7.5);


% \draw[black] (13,6) -- (13,6.75);
% \draw[black] (13,7.5) -- (13,6.75);
% \draw[red] (13,7.5) -- (13.75,7.5);
% \draw[black] (13.75,7.5) -- (13.75,8.25);
% \draw[red] (14.5,8.25) -- (13.75,8.25);
% \draw[red] (14.5,8.25) -- (15.25,8.25);
% \draw[black] (15.25,9) -- (15.25,8.25);
% \draw[red] (15.25,9) -- (16,9);
% \draw[black, dotted] (13,6) -- (16,9);

% \filldraw[white] (13,6) circle (1pt);
% \filldraw[white] (13,6.75) circle (1pt);
% \filldraw[white] (13,7.5) circle (1pt);
% \filldraw[white] (13.75,7.5) circle (1pt);
% \filldraw[white] (13.75,8.25) circle (1pt);
% \filldraw[white] (14.5,8.25) circle (1pt);
% \filldraw[white] (15.25,8.25) circle (1pt);
% \filldraw[white] (15.25,9) circle (1pt);
% \filldraw[white] (16,9) circle (1pt);






%%%% -------------------------------------------- %%%%%

% c(D)-ex1

% \draw[red] (1,1) -- (1,4);
% \draw[red] (1,4) -- (1.75,4);
% \draw[black] (1.75,4.75) -- (1.75,4);
% \draw[black] (1.75,4.75) -- (2.5,4.75);
% \draw[black] (2.5,5.5) -- (2.5,4.75);
% \draw[black] (2.5,5.5) -- (3.25,5.5);
% \draw[red] (4.75,5.5) -- (3.25,5.5);
% \draw[black] (4.75,5.5) -- (4.75,7);
% \draw[black] (6.25,7) -- (4.75,7);
% \draw[red] (6.25,7) -- (7,7);
% \draw[black] (7,7.75) -- (7,7);
% \draw[black] (7,7.75) -- (7.75,7.75);
% \draw[black, dotted] (1,1) -- (7.75,7.75);

% \filldraw[white] (1,1) circle (1pt);
% \filldraw[white] (1,1.75) circle (1pt);
% \filldraw[white] (1,2.5) circle (1pt);
% \filldraw[white] (1,3.25) circle (1pt);
% \filldraw[white] (1,4) circle (1pt);
% \filldraw[white] (1.75,4) circle (1pt);
% \filldraw[white] (1.75,4.75) circle (1pt);
% \filldraw[white] (2.5,4.75) circle (1pt);
% \filldraw[white] (2.5,5.5) circle (1pt);
% \filldraw[white] (3.25,5.5) circle (1pt);
% \filldraw[white] (4,5.5) circle (1pt);
% \filldraw[white] (4.75,5.5) circle (1pt);
% \filldraw[white] (4.75,6.25) circle (1pt);
% \filldraw[white] (4.75,7) circle (1pt);
% \filldraw[white] (5.5,7) circle (1pt);
% \filldraw[white] (6.25,7) circle (1pt);
% \filldraw[white] (7,7) circle (1pt);
% \filldraw[white] (7,7.75) circle (1pt);
% \filldraw[white] (7.75,7.75) circle (1pt);





%%%% -------------------------------------------- %%%%%

% c(D)-ex2

% \draw[red] (1,1) -- (1,3.25);
% \draw[black] (1,4) -- (1,3.25);
% \draw[black] (1,4) -- (1.75,4);
% \draw[black] (1.75,4.75) -- (1.75,4);
% \draw[black] (1.75,4.75) -- (2.5,4.75);
% \draw[black] (2.5,5.5) -- (2.5,4.75);
% \draw[black] (2.5,5.5) -- (3.25,5.5);
% \draw[red] (4.75,5.5) -- (3.25,5.5);
% \draw[black] (4.75,5.5) -- (4.75,7);
% \draw[black] (6.25,7) -- (4.75,7);
% \draw[red] (6.25,7) -- (7,7);
% \draw[black] (7,7.75) -- (7,7);
% \draw[black] (7,7.75) -- (7.75,7.75);
% \draw[black, dotted] (1,1) -- (7.75,7.75);

% \filldraw[white] (1,1) circle (1pt);
% \filldraw[white] (1,1.75) circle (1pt);
% \filldraw[white] (1,2.5) circle (1pt);
% \filldraw[white] (1,3.25) circle (1pt);
% \filldraw[white] (1,4) circle (1pt);
% \filldraw[white] (1.75,4) circle (1pt);
% \filldraw[white] (1.75,4.75) circle (1pt);
% \filldraw[white] (2.5,4.75) circle (1pt);
% \filldraw[white] (2.5,5.5) circle (1pt);
% \filldraw[white] (3.25,5.5) circle (1pt);
% \filldraw[white] (4,5.5) circle (1pt);
% \filldraw[white] (4.75,5.5) circle (1pt);
% \filldraw[white] (4.75,6.25) circle (1pt);
% \filldraw[white] (4.75,7) circle (1pt);
% \filldraw[white] (5.5,7) circle (1pt);
% \filldraw[white] (6.25,7) circle (1pt);
% \filldraw[white] (7,7) circle (1pt);
% \filldraw[white] (7,7.75) circle (1pt);
% \filldraw[white] (7.75,7.75) circle (1pt);










%%%% -------------------------------------------- %%%%%

% f_n,k-ex1


% \node (v17) [fill = white, circle, anchor=center] at (9,9) {17};
% \node (v16) [fill = white, circle, anchor=center] at (11,8) {16};
% \node (v15) [fill = white, circle, anchor=center] at (12,7) {15};
% \node (v14) [fill = white, circle, anchor=center] at (10,7) {14};
% \node (v13) [fill = white, circle, anchor=center] at (7,8) {\textcolor{red}{13}};
% \node (v12) [fill = white, circle, anchor=center] at (8,7) {12};
% \node (v11) [fill = white, circle, anchor=center] at (7,6) {\textcolor{red}{11}};
% \node (v10) [fill = white, circle, anchor=center] at (8,5) {\textcolor{red}{10}};
% \node (v9) [fill = white, circle, anchor=center] at (9,4) {9};
% \node (v8) [fill = white, circle, anchor=center] at (10,3) {8};
% \node (v7) [fill = white, circle, anchor=center] at (8,3) {7};
% \node (v6) [fill = white, circle, anchor=center] at (7,4) {\textcolor{blue}{6}};
% \node (v5) [fill = white, circle, anchor=center] at (9,2) {\textcolor{blue}{5}};
% \node (v4) [fill = white, circle, anchor=center] at (6,7) {\textcolor{blue}{4}};
% \node (v3) [fill = white, circle, anchor=center] at (7,2) {\textcolor{blue}{3}};
% \node (v2) [fill = white, circle, anchor=center] at (8,1) {\textcolor{blue}{2}};
% \node (v1) [fill = white, circle, anchor=center] at (5,6) {\textcolor{blue}{1}};


% \draw[black] (v17) -- (v16);
% \draw[black] (v14) -- (v16);
% \draw[black] (v15) -- (v16);
% \draw[black] (v17) -- (v13);
% \draw[black] (v12) -- (v13);
% \draw[black] (v12) -- (v11);
% \draw[black] (v10) -- (v11);
% \draw[black] (v10) -- (v9);
% \draw[black] (v10) -- (v6);
% \draw[black] (v7) -- (v9);
% \draw[black] (v8) -- (v9);
% \draw[black] (v7) -- (v5);
% \draw[black] (v4) -- (v13);
% \draw[black] (v4) -- (v1);
% \draw[black] (v7) -- (v3);
% \draw[black] (v2) -- (v3);









%%%% -------------------------------------------- %%%%%

% f_n,k-ex2

% \node [fill = none,scale=1,anchor=center] at (14,11) {$c(T) = (2,0,1,2,1)$};


% \node (v17) [fill = white, circle, anchor=center] at (9,9) {17};
% \node (v16) [fill = white, circle, anchor=center] at (11,8) {16};
% \node (v15) [fill = white, circle, anchor=center] at (12,7) {15};
% \node (v14) [fill = white, circle, anchor=center] at (10,7) {14};
% \node (v13) [fill = white, circle, anchor=center] at (7,8) {\textcolor{red}{13}};
% \node (v12) [fill = white, circle, anchor=center] at (15,9) {12};
% \node (v11) [fill = white, circle, anchor=center] at (14,8) {\textcolor{red}{11}};
% \node (v10) [fill = white, circle, anchor=center] at (17,9) {\textcolor{red}{10}};
% \node (v9) [fill = white, circle, anchor=center] at (20,9) {9};
% \node (v8) [fill = white, circle, anchor=center] at (21,8) {8};
% \node (v7) [fill = white, circle, anchor=center] at (19,8) {7};


% \draw[black] (v17) -- (v16);
% \draw[black] (v14) -- (v16);
% \draw[black] (v15) -- (v16);
% \draw[black] (v17) -- (v13);
% \draw[black] (v12) -- (v11);
% \draw[black] (v7) -- (v9);
% \draw[black] (v8) -- (v9);

% \node [fill = none,circle,scale=1,anchor=center] at (9,9.75) {$B_1$};
% \node [fill = none,circle,scale=1,anchor=center] at (15,9.75) {$B_2$};
% \node [fill = none,circle,scale=1,anchor=center] at (17,9.75) {$B_3$};
% \node [fill = none,circle,scale=1,anchor=center] at (20,9.75) {$B_4$};

% \node [fill = none,circle,scale=1,anchor=center] at (9,5.75) {$D_1$};
% \node [fill = none,circle,scale=1,anchor=center] at (15,5.75) {$D_2$};
% \node [fill = none,circle,scale=1,anchor=center] at (17,5.75) {$D_3$};
% \node [fill = none,circle,scale=1,anchor=center] at (20,5.75) {$D_4$};

% \draw[black] (7.125,1.25) -- (7.125,2.75);
% \draw[black] (7.875,2.75) -- (7.125,2.75);
% \draw[black] (7.875,2.75) -- (7.875,4.25);
% \draw[black] (9.375,4.25) -- (7.875,4.25);
% \draw[black] (9.375,4.25) -- (9.375,5);
% \draw[black] (10.875,5) -- (9.375,5);
% \draw[black, dotted] (10.875,5) -- (7.125,1.25);

% \filldraw[white] (7.125,1.25) circle (1pt);
% \filldraw[white] (7.125,2) circle (1pt);
% \filldraw[white] (7.125,2.75) circle (1pt);
% \filldraw[white] (7.875,2.75) circle (1pt);
% \filldraw[white] (7.875,3.5) circle (1pt);
% \filldraw[white] (7.875,4.25) circle (1pt);
% \filldraw[white] (8.625,4.25) circle (1pt);
% \filldraw[white] (9.375,4.25) circle (1pt);
% \filldraw[white] (9.375,5) circle (1pt);
% \filldraw[white] (10.125,5) circle (1pt);
% \filldraw[white] (10.875,5) circle (1pt);

% \draw[black] (14.25,3.5) -- (14.25,5);
% \draw[black] (15.75,5) -- (14.25,5);
% \draw[black, dotted] (15.75,5) -- (14.25,3.5);

% \filldraw[white] (14.25,3.5) circle (1pt);
% \filldraw[white] (14.25,4.25) circle (1pt);
% \filldraw[white] (14.25,5) circle (1pt);
% \filldraw[white] (15,5) circle (1pt);
% \filldraw[white] (15.75,5) circle (1pt);

% \draw[black] (16.625,4.25) -- (16.625,5);
% \draw[black] (17.375,5) -- (16.625,5);
% \draw[black, dotted] (17.375,5) -- (16.625,4.25);

% \filldraw[white] (16.625,4.25) circle (1pt);
% \filldraw[white] (16.625,5) circle (1pt);
% \filldraw[white] (17.375,5) circle (1pt);

% \draw[black] (18.875,2.75) -- (18.875,4.25);
% \draw[black] (19.625,4.25) -- (18.875,4.25);
% \draw[black] (19.625,4.25) -- (19.625,5);
% \draw[black] (21.125,5) -- (19.625,5);
% \draw[black, dotted] (21.125,5) -- (18.875,2.75);

% \filldraw[white] (18.875,2.75) circle (1pt);
% \filldraw[white] (18.875,3.5) circle (1pt);
% \filldraw[white] (18.875,4.25) circle (1pt);
% \filldraw[white] (19.625,4.25) circle (1pt);
% \filldraw[white] (19.625,5) circle (1pt);
% \filldraw[white] (20.375,5) circle (1pt);
% \filldraw[white] (21.125,5) circle (1pt);









%%%% -------------------------------------------- %%%%%

% f_n,k-ex3


% \draw[blue] (0,0) -- (0,4.5);
% \draw[blue] (0.75,4.5) -- (0,4.5);
% \draw[black] (0.75,4.5) -- (0.75,6);
% \draw[black] (1.5,6) -- (0.75,6);
% \draw[black] (1.5,6) -- (1.5,6.75);
% \draw[black] (3,6.75) -- (1.5,6.75);
% \draw[blue] (3,6.75) -- (4.5,6.75);
% \draw[black] (4.5,7.5) -- (4.5,6.75);
% \draw[black] (4.5,7.5) -- (5.25,7.5);
% \draw[blue] (6,7.5) -- (5.25,7.5);
% \draw[black] (6,7.5) -- (6,9);
% \draw[black] (7.5,9) -- (6,9);
% \draw[black] (7.5,9) -- (7.5,10.5);
% \draw[black] (8.25,10.5) -- (7.5,10.5);
% \draw[black] (8.25,10.5) -- (8.25,12);
% \draw[black] (9.75,12) -- (8.25,12);
% \draw[black] (9.75,12) -- (9.75,12.75);
% \draw[black] (11.25,12.75) -- (9.75,12.75);
% \draw[blue] (11.25,12.75) -- (12.75,12.75);
% \draw[black, dotted] (0,0) -- (12.75,12.75);

% \filldraw[white] (0,0) circle (1pt);
% \filldraw[white] (0,0.75) circle (1pt);
% \filldraw[white] (0,1.5) circle (1pt);
% \filldraw[white] (0,2.25) circle (1pt);
% \filldraw[white] (0,3) circle (1pt);
% \filldraw[white] (0,3.75) circle (1pt);
% \filldraw[white] (0,4.5) circle (1pt);
% \filldraw[white] (0.75,4.5) circle (1pt);
% \filldraw[white] (0.75,5.25) circle (1pt);
% \filldraw[white] (0.75,6) circle (1pt);
% \filldraw[white] (1.5,6) circle (1pt);
% \filldraw[white] (1.5,6.75) circle (1pt);
% \filldraw[white] (2.25,6.75) circle (1pt);
% \filldraw[white] (3,6.75) circle (1pt);
% \filldraw[white] (3.75,6.75) circle (1pt);
% \filldraw[white] (4.5,6.75) circle (1pt);
% \filldraw[white] (4.5,7.5) circle (1pt);
% \filldraw[white] (5.25,7.5) circle (1pt);
% \filldraw[white] (6,7.5) circle (1pt);
% \filldraw[white] (6,8.25) circle (1pt);
% \filldraw[white] (6,9) circle (1pt);
% \filldraw[white] (6.75,9) circle (1pt);
% \filldraw[white] (7.5,9) circle (1pt);
% \filldraw[white] (7.5,9.75) circle (1pt);
% \filldraw[white] (7.5,10.5) circle (1pt);
% \filldraw[white] (8.25,10.5) circle (1pt);
% \filldraw[white] (8.25,11.25) circle (1pt);
% \filldraw[white] (8.25,12) circle (1pt);
% \filldraw[white] (9,12) circle (1pt);
% \filldraw[white] (9.75,12) circle (1pt);
% \filldraw[white] (9.75,12.75) circle (1pt);
% \filldraw[white] (10.5,12.75) circle (1pt);
% \filldraw[white] (11.25,12.75) circle (1pt);
% \filldraw[white] (12,12.75) circle (1pt);
% \filldraw[white] (12.75,12.75) circle (1pt);

% \node [fill = none,scale=1,anchor=center] at (6,12.75) {$D$};
% \node [fill = none,scale=1,anchor=center] at (6,13.5) {$\omega = 146325$};










%%%% -------------------------------------------- %%%%%

% A-L-ex


% \node (v8) [fill = black, circle, anchor=center] at (6,10) {};
% \node (v7) [fill = black, circle, anchor=center] at (8,10) {};
% \node (v6) [fill = black, circle, anchor=center] at (4,10) {};
% \node (v5) [fill = black, circle, anchor=center] at (6,8) {};
% \node (v4) [fill = black, circle, anchor=center] at (6,6) {};
% \node (v3) [fill = black, circle, anchor=center] at (6,4) {};
% \node (v2) [fill = black, circle, anchor=center] at (6,2) {};
% \node (v1) [fill = black, circle, anchor=center] at (6,0) {};

% \draw[black, thick] (v1) -- (v2);
% \draw[black, thick] (v3) -- (v2);
% \draw[black, thick] (v3) -- (v4);
% \draw[black, thick] (v4) -- (v5);
% \draw[black, thick] (v5) -- (v6);
% \draw[black, thick] (v5) -- (v7);
% \draw[black, thick] (v5) -- (v8);

% \node [fill = none, anchor=center, scale = 1.5] at (5.75,1) {$1$};
% \node [fill = none, anchor=center, scale = 1.5] at (5.75,3) {$2$};
% \node [fill = none, anchor=center, scale = 1.5] at (5.75,5) {$3$};
% \node [fill = none, anchor=center, scale = 1.5] at (5.75,7) {$4$};
% \node [fill = none, anchor=center, scale = 1.5] at (5.75,9) {$5$};
% \node [fill = none, anchor=center, scale = 1.5] at (4.75,8.75) {$6$};
% \node [fill = none, anchor=center, scale = 1.5] at (7.25,8.75) {$7$};

% \node [fill = white, anchor=center, scale = 2] at (6,-1.5) {$A_{4,3}$};



% \node (v1) [fill = black, circle, anchor=center] at (14,1) {};
% \node (v2) [fill = black, circle, anchor=center] at (14,3) {};
% \node (v3) [fill = black, circle, anchor=center] at (14,5) {};
% \node (v4) [fill = blue, circle, anchor=center] at (14,7) {};
% \node (v5) [fill = red, circle, anchor=center] at (12.5,8.5) {};
% \node (v6) [fill = red, circle, anchor=center] at (15.5,8.5) {};
% \node (v7) [fill = red, circle, anchor=center] at (14,10) {};

% \draw[black, thick] (v1) -- (v2);
% \draw[black, thick] (v3) -- (v2);
% \draw[black, thick] (v3) -- (v4);
% \draw[black, thick] (v5) -- (v4);
% \draw[black, thick] (v6) -- (v4);
% \draw[black, thick] (v7) -- (v4);
% \draw[black, thick] (v5) -- (v6);
% \draw[black, thick] (v5) -- (v7);
% \draw[black, thick] (v6) -- (v7);

% \node [fill = none, anchor=center, scale = 1.5] at (13.5,1) {$1$};
% \node [fill = none, anchor=center, scale = 1.5] at (13.5,3) {$2$};
% \node [fill = none, anchor=center, scale = 1.5] at (13.5,5) {$3$};
% \node [fill = none, anchor=center, scale = 1.5] at (13.5,7) {$4$};
% \node [fill = none, anchor=center, scale = 1.5] at (13.5,10) {$5$};
% \node [fill = none, anchor=center, scale = 1.5] at (12,8.5) {$6$};
% \node [fill = none, anchor=center, scale = 1.5] at (16,8.5) {$7$};

% \node [fill = white, anchor=center, scale = 2] at (14,-1.5) {$L_{3,4}$};
















%%%% -------------------------------------------- %%%%%

% v-ex



% \node (v8) [fill = white, circle, anchor=center] at (5,6) {8};
% \node (v7) [fill = white, circle, anchor=center] at (6,5) {7};
% \node (v6) [fill = white, circle, anchor=center] at (5.5,4) {6};
% \node (v5) [fill = white, circle, anchor=center] at (4,5) {5};
% \node (v4) [fill = white, circle, anchor=center] at (4.5,4) {4};
% \node (v3) [fill = white, circle, anchor=center] at (3.5,4) {3};
% \node (v2) [fill = white, circle, anchor=center] at (4,3) {2};
% \node (v1) [fill = white, circle, anchor=center] at (3.5,2) {1};

% \draw[black] (v8) -- (v7);
% \draw[black] (v6) -- (v7);
% \draw[black] (v8) -- (v5);
% \draw[black] (v4) -- (v5);
% \draw[black] (v3) -- (v5);
% \draw[red] (v3) -- (v2);
% \draw[red] (v1) -- (v2);


% \node (v8) [fill = white, circle, anchor=center] at (10,6) {6};
% \node (v7) [fill = white, circle, anchor=center] at (11,5) {5};
% \node (v6) [fill = white, circle, anchor=center] at (10.5,4) {4};
% \node (v5) [fill = white, circle, anchor=center] at (9,5) {3};
% \node (v4) [fill = white, circle, anchor=center] at (9.5,4) {1};
% \node (v3) [fill = white, circle, anchor=center] at (8.5,4) {2};
% \node (v2) [fill = white, circle, anchor=center] at (9.5,7) {7};
% \node (v1) [fill = white, circle, anchor=center] at (10,8) {8};

% \draw[black] (v8) -- (v7);
% \draw[black] (v6) -- (v7);
% \draw[black] (v8) -- (v5);
% \draw[black] (v4) -- (v5);
% \draw[black] (v3) -- (v5);
% \draw[red] (v8) -- (v2);
% \draw[red] (v1) -- (v2);


% \draw[-Stealth, black] (6.5,5) -- (8,5);
% \node [fill = none, anchor=center] at (7.25,5.25) {$\varphi$};














%%%% -------------------------------------------- %%%%%

% tubing-to-B

% \node (v1) [fill = white, circle, anchor=center, scale = 0.75] at (0,1) {1};
% \node (v2) [fill = white, circle, anchor=center, scale = 0.75] at (0,2) {2};
% \node (v3) [fill = white, circle, anchor=center, scale = 0.75] at (0,3) {3};
% \node (v4) [fill = white, circle, anchor=center, scale = 0.75] at (0,4) {4};
% \node (v5) [fill = white, circle, anchor=center, scale = 0.75] at (0,5) {5};
% \node (v6) [fill = white, circle, anchor=center, scale = 0.75] at (0,6) {6};
% \node (v7) [fill = white, circle, anchor=center, scale = 0.75] at (0,7) {7};
% \node (v8) [fill = white, circle, anchor=center, scale = 0.75] at (0,8) {8};
% \node (v9) [fill = white, circle, anchor=center, scale = 0.75] at (0,9) {9};
% \node (v10) [fill = white, circle, anchor=center, scale = 0.75] at (0,10) {10};
% \node (v11) [fill = white, circle, anchor=center, scale = 0.75] at (0,11) {11};
% \node (v12) [fill = white, circle, anchor=center, scale = 0.75] at (0,12) {12};
% \node (v13) [fill = white, circle, anchor=center, scale = 0.75] at (-1,13) {13};
% \node (v14) [fill = white, circle, anchor=center, scale = 0.75] at (1,13) {14};
% \node (v15) [fill = white, circle, anchor=center, scale = 0.75] at (0,14) {15};

% \draw[black] (v1) -- (v2);
% \draw[black] (v2) -- (v3);
% \draw[black] (v3) -- (v4);
% \draw[black] (v4) -- (v5);
% \draw[black] (v5) -- (v6);
% \draw[black] (v6) -- (v7);
% \draw[black] (v7) -- (v8);
% \draw[black] (v8) -- (v9);
% \draw[black] (v9) -- (v10);
% \draw[black] (v10) -- (v11);
% \draw[black] (v11) -- (v12);
% \draw[black] (v12) -- (v13);
% \draw[black] (v12) -- (v14);
% \draw[black] (v12) -- (v15);
% \draw[black] (v13) -- (v14);
% \draw[black] (v13) -- (v15);
% \draw[black] (v14) -- (v15);


% \draw (v11) [red] circle (0.2cm) [fill=none];
% \draw[red] \convexpath{v11,v12}{0.25cm};
% \draw[red] \convexpath{v11,v12,v14}{0.3cm};

% \draw (v7) [red] circle (0.2cm) [fill=none];
% \draw (v9) [red] circle (0.2cm) [fill=none];
% \draw[red] \convexpath{v7,v9}{0.25cm};
% \draw[red] \convexpath{v7,v12,v14}{0.35cm};
% \draw[red] \convexpath{v6,v12,v14}{0.4cm};

% \draw (v4) [red] circle (0.2cm) [fill=none];
% \draw[red] \convexpath{v4,v12,v14}{0.5cm};
% \draw[red] \convexpath{v4,v15,v14}{0.6cm};
% \draw[red] \convexpath{v4,v13,v15,v14}{0.7cm};

% \draw (v2) [red] circle (0.2cm) [fill=none];
% \draw[red] \convexpath{v1,v2}{0.25cm};


% \node (t1) [fill = white, circle, anchor=center, scale = 0.75] at (8,11) {1};
% \node (t2) [fill = white, circle, anchor=center, scale = 0.75] at (8,10) {2};
% \node (t3) [fill = white, circle, anchor=center, scale = 0.75] at (7,12) {\textcolor{blue}{3}};
% \node (t4) [fill = white, circle, anchor=center, scale = 0.75, scale = 0.75] at (7,8) {4};
% \node (t5) [fill = white, circle, anchor=center, scale = 0.75] at (6,9) {\textcolor{blue}{5}};
% \node (t6) [fill = white, circle, anchor=center, scale = 0.75] at (5,8) {\textcolor{blue}{6}};
% \node (t7) [fill = white, circle, anchor=center, scale = 0.75] at (5.5,5) {7};
% \node (t8) [fill = white, circle, anchor=center, scale = 0.75] at (6,6) {8};
% \node (t9) [fill = white, circle, anchor=center, scale = 0.75] at (6.5,5) {9};
% \node (t10) [fill = white, circle, anchor=center, scale = 0.75] at (5,7) {\textcolor{blue}{10}};
% \node (t11) [fill = white, circle, anchor=center, scale = 0.75] at (4,4) {11};
% \node (t12) [fill = white, circle, anchor=center, scale = 0.75] at (4,5) {12};
% \node (t13) [fill = white, circle, anchor=center, scale = 0.75] at (6,11) {\textcolor{red}{13}};
% \node (t14) [fill = white, circle, anchor=center, scale = 0.75] at (4,6) {\textcolor{red}{14}};
% \node (t15) [fill = white, circle, anchor=center, scale = 0.75] at (6,10) {\textcolor{red}{15}};

% \draw[black] (t11) -- (t12);
% \draw[black] (t14) -- (t12);
% \draw[black] (t14) -- (t10);
% \draw[black] (t8) -- (t10);
% \draw[black] (t8) -- (t7);
% \draw[black] (t8) -- (t9);
% \draw[black] (t6) -- (t10);
% \draw[black] (t6) -- (t5);
% \draw[black] (t4) -- (t5);
% \draw[black] (t15) -- (t5);
% \draw[black] (t15) -- (t13);
% \draw[black] (t3) -- (t13);
% \draw[black] (t3) -- (t1);
% \draw[black] (t2) -- (t1);






%%%% -------------------------------------------- %%%%%

% degrading


% \node (v1) [fill = black, circle, anchor=center, scale = 0.5] at (0,10) {};
% \node (v2) [fill = black, circle, anchor=center, scale = 0.5] at (0,9) {};
% \node (v3) [fill = red, circle, anchor=center, scale = 0.5] at (0,8) {};
% \node (v4) [fill = red, circle, anchor=center, scale = 0.5] at (0,7) {};
% \node (v5) [fill = black, circle, anchor=center, scale = 0.5] at (0,6) {};
% \node (v6) [fill = black, circle, anchor=center, scale = 0.5] at (0,5) {};
% \node (v7) [fill = black, circle, anchor=center, scale = 0.5] at (0,4) {};
% \node (v8) [fill = black, circle, anchor=center, scale = 0.5] at (0,3) {};
% \node (v9) [fill = black, circle, anchor=center, scale = 0.5] at (0,2) {};
% \node (v10) [fill = black, circle, anchor=center, scale = 0.5] at (0,1) {};

% \draw[black] (v1) -- (v2);
% \draw[black] (v2) -- (v3);
% \draw[black] (v3) -- (v4);
% \draw[black] (v4) -- (v5);
% \draw[black] (v5) -- (v6);
% \draw[black] (v6) -- (v7);
% \draw[black] (v7) -- (v8);
% \draw[black] (v8) -- (v9);
% \draw[black] (v9) -- (v10);

% \draw[red] \convexpath{v1,v2}{0.25cm};
% \draw[blue] \convexpath{v5,v6}{0.25cm};
% \draw[red] \convexpath{v5,v7}{0.35cm};
% \draw[red] \convexpath{v8,v10}{0.25cm};






%%%% -------------------------------------------- %%%%%

% degrade-to-nondegrade

% \node (v1) [fill = black, circle, anchor=center, scale = 0.5] at (-1,8) {};
% \node (v2) [fill = black, circle, anchor=center, scale = 0.5] at (0,8) {};
% \node (v3) [fill = black, circle, anchor=center, scale = 0.5] at (1,8) {};
% \node (v4) [fill = blue, circle, anchor=center, scale = 0.5] at (0,7) {};
% \node (v5) [fill = blue, circle, anchor=center, scale = 0.5] at (0,6) {};
% \node (v6) [fill = blue, circle, anchor=center, scale = 0.5] at (0,5) {};
% \node (v7) [fill = blue, circle, anchor=center, scale = 0.5] at (0,4) {};
% \node (v8) [fill = blue, circle, anchor=center, scale = 0.5] at (0,3) {};
% \node (v9) [fill = black, circle, anchor=center, scale = 0.5] at (-0.5,2) {};
% \node (v10) [fill = black, circle, anchor=center, scale = 0.5] at (0.5,2) {};

% \draw[black] (v1) -- (v4);
% \draw[black] (v2) -- (v4);
% \draw[black] (v3) -- (v4);
% \draw[blue] (v4) -- (v5);
% \draw[blue] (v5) -- (v6);
% \draw[blue] (v6) -- (v7);
% \draw[blue] (v7) -- (v8);
% \draw[black] (v8) -- (v9);
% \draw[black] (v8) -- (v10);

% \draw[blue] \convexpath{v4,v5}{0.2cm};
% \draw[blue] \convexpath{v6,v7}{0.2cm};
% \draw[red] \convexpath{v1,v2,v5}{0.25cm};
% \draw[red] \convexpath{v10,v8}{0.2cm};
% \draw[red] \convexpath{v9,v6,v10}{0.25cm};

% \node (v1) [fill = black, circle, anchor=center, scale = 0.5] at (4,7) {};
% \node (v2) [fill = black, circle, anchor=center, scale = 0.5] at (5,7) {};
% \node (v3) [fill = black, circle, anchor=center, scale = 0.5] at (6,7) {};
% \node (v5) [fill = blue, circle, anchor=center, scale = 0.5] at (5,6) {};
% \node (v6) [fill = blue, circle, anchor=center, scale = 0.5] at (5,5) {};
% \node (v8) [fill = blue, circle, anchor=center, scale = 0.5] at (5,4) {};
% \node (v9) [fill = black, circle, anchor=center, scale = 0.5] at (4.5,3) {};
% \node (v10) [fill = black, circle, anchor=center, scale = 0.5] at (5.5,3) {};

% \draw[black] (v1) -- (v5);
% \draw[black] (v2) -- (v5);
% \draw[black] (v3) -- (v5);
% \draw[blue] (v5) -- (v6);
% \draw[blue] (v6) -- (v8);
% \draw[black] (v8) -- (v9);
% \draw[black] (v8) -- (v10);

% \draw[red] \convexpath{v1,v2,v5}{0.25cm};
% \draw[red] \convexpath{v10,v8}{0.2cm};
% \draw[red] \convexpath{v9,v6,v10}{0.25cm};






%%%% -------------------------------------------- %%%%%

% brooms

% \node (v1) [fill = black, circle, anchor=center, scale = 0.5] at (-1,8) {};
% \node (v2) [fill = black, circle, anchor=center, scale = 0.5] at (0,8) {};
% \node (v3) [fill = black, circle, anchor=center, scale = 0.5] at (1,8) {};
% \node (v4) [fill = black, circle, anchor=center, scale = 0.5] at (0,7) {};

% \draw[black] (v1) -- (v4);
% \draw[black] (v2) -- (v4);
% \draw[black] (v3) -- (v4);

% \node [anchor=center, scale = 1] at (0,4) {$A_{0,3}$};

% \node (v1) [fill = black, circle, anchor=center, scale = 0.5] at (3,8) {};
% \node (v2) [fill = black, circle, anchor=center, scale = 0.5] at (4,8) {};
% \node (v3) [fill = black, circle, anchor=center, scale = 0.5] at (5,8) {};
% \node (v5) [fill = black, circle, anchor=center, scale = 0.5] at (4,7) {};
% \node (v6) [fill = black, circle, anchor=center, scale = 0.5] at (4,6) {};
% \node (v8) [fill = black, circle, anchor=center, scale = 0.5] at (4,5) {};

% \draw[black] (v1) -- (v5);
% \draw[black] (v2) -- (v5);
% \draw[black] (v3) -- (v5);
% \draw[black] (v5) -- (v6);
% \draw[black] (v6) -- (v8);

% \node [anchor=center, scale = 1] at (4,4) {$A_{2,3}$};

% \node (v2) [fill = black, circle, anchor=center, scale = 0.5] at (8,8) {};
% \node (v5) [fill = black, circle, anchor=center, scale = 0.5] at (8,7) {};
% \node (v6) [fill = black, circle, anchor=center, scale = 0.5] at (8,6) {};
% \node (v8) [fill = black, circle, anchor=center, scale = 0.5] at (8,5) {};

% \draw[black] (v2) -- (v5);
% \draw[black] (v5) -- (v6);
% \draw[black] (v6) -- (v8);

% \node [anchor=center, scale = 1] at (8,4) {$A_{3,0}$};









%%%% -------------------------------------------- %%%%%

% DCEx


% \coordinate (s1) at (0,{8*sqrt(3)+11.5});
% \coordinate (s2) at ({0+sqrt(3)*3/4},{8*sqrt(3)+9.25});
% \coordinate (s3) at ({0-sqrt(3)*3/4},{8*sqrt(3)+9.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s2,s1}{0.4cm};

% \coordinate (s1) at (0,{8*sqrt(3)+6.5});
% \coordinate (s2) at ({0+sqrt(3)*3/4},{8*sqrt(3)+4.25});
% \coordinate (s3) at ({0-sqrt(3)*3/4},{8*sqrt(3)+4.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s1,s3}{0.4cm};

% \coordinate (s1) at (0,{8*sqrt(3)+1.5});
% \coordinate (s2) at ({0+sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s3) at ({0-sqrt(3)*3/4},{8*sqrt(3)-0.75});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s2,s3}{0.4cm};





% \coordinate (s1) at (5,{8*sqrt(3)+11.5});
% \coordinate (s2) at ({5+sqrt(3)*3/4},{8*sqrt(3)+9.25});
% \coordinate (s3) at ({5-sqrt(3)*3/4},{8*sqrt(3)+9.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s1) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at (5,{8*sqrt(3)+6.5});
% \coordinate (s2) at ({5+sqrt(3)*3/4},{8*sqrt(3)+4.25});
% \coordinate (s3) at ({5-sqrt(3)*3/4},{8*sqrt(3)+4.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s2) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at (5,{8*sqrt(3)+1.5});
% \coordinate (s2) at ({5+sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s3) at ({5-sqrt(3)*3/4},{8*sqrt(3)-0.75});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s3) [red] circle (0.4cm) [fill=none];








% \coordinate (s1) at (10,{8*sqrt(3)+11.5});
% \coordinate (s2) at ({10+sqrt(3)*3/4},{8*sqrt(3)+9.25});
% \coordinate (s3) at ({10-sqrt(3)*3/4},{8*sqrt(3)+9.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s2,s1}{0.4cm};

% \coordinate (s1) at (10,{8*sqrt(3)+6.5});
% \coordinate (s2) at ({10+sqrt(3)*3/4},{8*sqrt(3)+4.25});
% \coordinate (s3) at ({10-sqrt(3)*3/4},{8*sqrt(3)+4.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s1,s3}{0.4cm};

% \coordinate (s1) at (10,{8*sqrt(3)+1.5});
% \coordinate (s2) at ({10+sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s3) at ({10-sqrt(3)*3/4},{8*sqrt(3)-0.75});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s2,s3}{0.4cm};





% \coordinate (s1) at (15,{8*sqrt(3)+11.5});
% \coordinate (s2) at ({15+sqrt(3)*3/4},{8*sqrt(3)+9.25});
% \coordinate (s3) at ({15-sqrt(3)*3/4},{8*sqrt(3)+9.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s1) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at (15,{8*sqrt(3)+6.5});
% \coordinate (s2) at ({15+sqrt(3)*3/4},{8*sqrt(3)+4.25});
% \coordinate (s3) at ({15-sqrt(3)*3/4},{8*sqrt(3)+4.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s2) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at (15,{8*sqrt(3)+1.5});
% \coordinate (s2) at ({15+sqrt(3)*3/4},{8*sqrt(3)-0.75});
% \coordinate (s3) at ({15-sqrt(3)*3/4},{8*sqrt(3)-0.75});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s3) [red] circle (0.4cm) [fill=none];









%%%% -------------------------------------------- %%%%%

% DPEx

% \coordinate (s1) at (0,{8*sqrt(3)+11.5});
% \coordinate (s2) at ({0},{8*sqrt(3)+13.75});
% \coordinate (s3) at ({0},{8*sqrt(3)+9.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[red] \convexpath{s2,s1}{0.4cm};

% \coordinate (s1) at (0,{8*sqrt(3)+7.625});
% \coordinate (s2) at ({0},{8*sqrt(3)+3.125});
% \coordinate (s3) at ({0},{8*sqrt(3)+5.375});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s1,s3}{0.4cm};

% \coordinate (s1) at (0,{8*sqrt(3)-3});
% \coordinate (s2) at ({0},{8*sqrt(3)-0.75});
% \coordinate (s3) at ({0},{8*sqrt(3)+1.5});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s2,s3}{0.4cm};





% \coordinate (s1) at ({5-sqrt(3)*2/4},{8*sqrt(3)+12.625});
% \coordinate (s2) at ({5+sqrt(3)*2/4},{8*sqrt(3)+10.375});
% \coordinate (s3) at ({5-sqrt(3)*2/4},{8*sqrt(3)+10.375});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw (s1) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at ({5-sqrt(3)*2/4},{8*sqrt(3)+4.25});
% \coordinate (s2) at ({5-sqrt(3)*2/4}, {8*sqrt(3)+6.5});
% \coordinate (s3) at ({5+sqrt(3)*2/4},{8*sqrt(3)+4.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw (s2) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at ({5+sqrt(3)*2/4},{8*sqrt(3)-1.825});
% \coordinate (s2) at ({5-sqrt(3)*2/4},{8*sqrt(3)-1.825});
% \coordinate (s3) at ({5-sqrt(3)*2/4},{8*sqrt(3)+0.375});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {2};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s3) [red] circle (0.4cm) [fill=none];







% \coordinate (s1) at (10,{8*sqrt(3)+11.5});
% \coordinate (s2) at ({10},{8*sqrt(3)+13.75});
% \coordinate (s3) at ({10},{8*sqrt(3)+9.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[red] \convexpath{s2,s1}{0.4cm};

% \coordinate (s1) at (10,{8*sqrt(3)+7.625});
% \coordinate (s2) at ({10},{8*sqrt(3)+3.125});
% \coordinate (s3) at ({10},{8*sqrt(3)+5.375});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s1,s3}{0.4cm};

% \coordinate (s1) at (10,{8*sqrt(3)-3});
% \coordinate (s2) at ({10},{8*sqrt(3)-0.75});
% \coordinate (s3) at ({10},{8*sqrt(3)+1.5});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[red] \convexpath{s2,s3}{0.4cm};





% \coordinate (s1) at ({15-sqrt(3)*2/4},{8*sqrt(3)+12.625});
% \coordinate (s2) at ({15+sqrt(3)*2/4},{8*sqrt(3)+10.375});
% \coordinate (s3) at ({15-sqrt(3)*2/4},{8*sqrt(3)+10.375});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n1);
% \draw (s1) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at ({15-sqrt(3)*2/4},{8*sqrt(3)+4.25});
% \coordinate (s2) at ({15-sqrt(3)*2/4}, {8*sqrt(3)+6.5});
% \coordinate (s3) at ({15+sqrt(3)*2/4},{8*sqrt(3)+4.25});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw (s2) [red] circle (0.4cm) [fill=none];

% \coordinate (s1) at ({15+sqrt(3)*2/4},{8*sqrt(3)-1.825});
% \coordinate (s2) at ({15-sqrt(3)*2/4},{8*sqrt(3)-1.825});
% \coordinate (s3) at ({15-sqrt(3)*2/4},{8*sqrt(3)+0.375});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {1};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {3};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {2};

% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw (s3) [red] circle (0.4cm) [fill=none];









%%%% -------------------------------------------- %%%%%

% tube-bijection

% \coordinate (s1) at ({0},{4});
% \coordinate (s2) at ({4 - 2*sqrt(2)},{4+2*sqrt(2)});
% \coordinate (s3) at ({4},{8});
% \coordinate (s4) at ({4 + 2*sqrt(2)},{4+2*sqrt(2)});
% \coordinate (s5) at ({8},{4});
% \coordinate (s6) at ({4 + 2*sqrt(2)},{4-2*sqrt(2)});
% \coordinate (s7) at ({4},{0});
% \coordinate (s8) at ({4 - 2*sqrt(2)},{4-2*sqrt(2)});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 10};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {\huge 7};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {\huge 1};
% \node (n4) [fill = white, circle, scale=1.5, anchor=center] at (s4) {\huge 8};
% \node (n5) [fill = white, circle, scale=1.5, anchor=center] at (s5) {\huge 4};
% \node (n6) [fill = white, circle, scale=1.5, anchor=center] at (s6) {\huge 13};
% \node (n7) [fill = white, circle, scale=1.5, anchor=center] at (s7) {\huge 14};
% \node (n8) [fill = white, circle, scale=1.5, anchor=center] at (s8) {\huge 3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n4);
% \draw[black, arrows = {-Stealth[scale=2]}] (n4) -- (n5);
% \draw[black, arrows = {-Stealth[scale=2]}] (n5) -- (n6);
% \draw[black, arrows = {-Stealth[scale=2]}] (n6) -- (n7);
% \draw[black, arrows = {-Stealth[scale=2]}] (n7) -- (n8);
% \draw[black, arrows = {-Stealth[scale=2]}] (n8) -- (n1);

% \draw[red] \convexpath{s1,s2,s3}{0.8cm};
% \draw[red] \convexpath{s2,s3}{0.6cm};
% \draw[red] \convexpath{s7,s6}{0.8cm};



% \coordinate (s1) at ({12},{6});
% \coordinate (s2) at ({16},{6});
% \coordinate (s3) at ({16},{2});
% \coordinate (s4) at ({12},{2});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 2};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {\huge 15};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {\huge 5};
% \node (n4) [fill = white, circle, scale=1.5, anchor=center] at (s4) {\huge 9};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[black, arrows = {-Stealth[scale=2]}] (n3) -- (n4);
% \draw[black, arrows = {-Stealth[scale=2]}] (n4) -- (n1);

% \draw[red] \convexpath{s1,s2,s3}{0.8cm};
% \draw (s1) [red] circle (0.6cm) [fill=none];
% \draw (s3) [red] circle (0.6cm) [fill=none];



% \coordinate (s1) at ({20},{4});
% \coordinate (s2) at ({24},{4});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 6};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {\huge 11};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) to[bend left] (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) to[bend left] (n1);


% \coordinate (s1) at ({28},{4});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 12};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) to[out=60,in=120,loop] (n1);







% \coordinate (s1) at ({2},{-16});
% \coordinate (s2) at ({2},{-12});
% \coordinate (s3) at ({2},{-8});
% \coordinate (s4) at ({18},{-14});
% \coordinate (s5) at ({10},{-18});
% \coordinate (s6) at ({10},{-14});
% \coordinate (s7) at ({10},{-10});
% \coordinate (s8) at ({2},{-20});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 10};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {\huge 7};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {\huge 1};
% \node (n4) [fill = white, circle, scale=1.5, anchor=center] at (s4) {\huge 8};
% \node (n5) [fill = white, circle, scale=1.5, anchor=center] at (s5) {\huge 4};
% \node (n6) [fill = white, circle, scale=1.5, anchor=center] at (s6) {\huge 13};
% \node (n7) [fill = white, circle, scale=1.5, anchor=center] at (s7) {\huge 14};
% \node (n8) [fill = white, circle, scale=1.5, anchor=center] at (s8) {\huge 3};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[black, arrows = {-Stealth[scale=2]}] (n5) -- (n6);
% \draw[black, arrows = {-Stealth[scale=2]}] (n6) -- (n7);
% \draw[black, arrows = {-Stealth[scale=2]}] (n8) -- (n1);

% \draw[red] \convexpath{s1,s3}{0.8cm};
% \draw[red] \convexpath{s3,s2}{0.6cm};
% \draw[red] \convexpath{s7,s6}{0.8cm};



% \coordinate (s1) at ({6},{-16});
% \coordinate (s2) at ({6},{-12});
% \coordinate (s3) at ({6},{-8});
% \coordinate (s4) at ({6},{-20});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 2};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {\huge 15};
% \node (n3) [fill = white, circle, scale=1.5, anchor=center] at (s3) {\huge 5};
% \node (n4) [fill = white, circle, scale=1.5, anchor=center] at (s4) {\huge 9};

% \draw[black, arrows = {-Stealth[scale=2]}] (n1) -- (n2);
% \draw[black, arrows = {-Stealth[scale=2]}] (n2) -- (n3);
% \draw[black, arrows = {-Stealth[scale=2]}] (n4) -- (n1);

% \draw[red] \convexpath{s1,s3}{0.8cm};
% \draw (s1) [red] circle (0.6cm) [fill=none];
% \draw (s3) [red] circle (0.6cm) [fill=none];



% \coordinate (s1) at ({14},{-14});
% \coordinate (s2) at ({22},{-14});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 6};
% \node (n2) [fill = white, circle, scale=1.5, anchor=center] at (s2) {\huge 11};


% \coordinate (s1) at ({26},{-14});

% \node (n1) [fill = white, circle, scale=1.5, anchor=center] at (s1) {\huge 12};


% \node (n1) [fill = white, scale=1.5, anchor=center] at (14,-6) {\huge $\sigma = (153)(2)(46)(7)$};

% \draw[black, arrows = {-Stealth[scale=2]}] (14,-2) -- (14, -4.5);
